Multi-agent Reinforcement Learning for Robotized Coral Reef Sample Collection

This paper presents a reinforcement learning (RL) environment for developing an autonomous underwater robotic coral sampling agent, a crucial coral reef conservation and research task. Using software-in-the-loop (SIL) and hardware-in-the-loop (HIL), an RL-trained artificial intelligence (AI) controller is developed using a digital twin (DT) in simulation and subsequently verified in physical experiments. An underwater motion capture (MOCAP) system provides real-time 3D position and orientation feedback during verification testing for precise synchronization between the digital and physical domains. A key novelty of this approach is the combined use of a general-purpose game engine for simulation, deep RL, and real-time underwater motion capture for an effective zero-shot sim-to-real strategy.

==> Datasets/large_scale_reward.tex <==
40000,-0.175255104899406
80000,-1.81333529949188
120000,4.17864751815796
160000,3.95817828178406
200000,7.25374937057495
240000,10.7722244262695
280000,4.68874311447144
320000,3.94840860366821
360000,9.88822841644287
400000,3.87867999076843
440000,9.32998371124268
480000,11.2633695602417
520000,16.7203006744385
560000,12.6720685958862
600000,15.5807247161865
640000,20.4217395782471
680000,21.1769599914551
720000,17.2313861846924
760000,14.1327037811279
800000,17.961706161499
840000,15.4961776733398
880000,19.5029392242432
920000,20.681661605835
960000,21.3342266082764
1000000,22.4739437103272
1040000,31.1529693603516
1080000,25.5816287994385
1120000,35.6453971862793
1160000,26.7408027648926
1200000,30.0764083862305
1240000,26.7438812255859
1280000,29.5601215362549
1320000,21.8371601104736
1360000,2.9735643863678
1400000,34.726619720459
1440000,29.8150844573975
1480000,19.5522155761719
1520000,21.8469905853272
1560000,22.2891235351563
1600000,27.3271770477295
1640000,32.3514938354492
1680000,21.9768257141113
1720000,20.9876766204834
1760000,39.7155075073242
1800000,42.2094497680664
1840000,42.3212471008301
1880000,71.6838302612305
1920000,66.6521072387695
1960000,72.8738403320313
2000000,70.2736511230469
2040000,68.4031829833984
2080000,70.1618881225586
2120000,74.9814834594727
2160000,69.65185546875
2200000,77.9379959106445
2240000,61.0272674560547
2280000,69.2977828979492
2320000,66.5905151367188
2360000,83.7781219482422
2400000,80.3392486572266
2440000,75.6702651977539
2480000,73.7829818725586
2520000,64.9375152587891
2560000,75.7366714477539
2600000,77.3210067749023
2640000,83.0921936035156
2680000,87.3118286132813
2720000,74.445426940918
2760000,83.5000610351563
2800000,97.1422424316406
2840000,96.6027145385742
2880000,85.7370071411133
2920000,72.6567230224609
2960000,67.849250793457
3000000,85.9949035644531
3040000,87.6502151489258
3080000,95.569465637207
3120000,91.0352783203125
3160000,104.67391204834
3200000,108.531112670898
3240000,84.2119064331055
3280000,79.640266418457
3320000,88.5413970947266
3360000,99.721435546875
3400000,95.1530227661133
3440000,102.383186340332
3480000,90.8411331176758
3520000,109.992309570313
3560000,95.839469909668
3600000,85.5849761962891
3640000,104.523773193359
3680000,86.3566207885742
3720000,98.0577697753906
3760000,75.4462127685547
3800000,93.0922546386719
3840000,116.613403320313
3880000,97.5794906616211
3920000,110.030944824219
3960000,101.41674041748
4000000,100.407485961914
4040000,117.426445007324
4080000,116.461029052734
4120000,106.501358032227
4160000,92.8746795654297
4200000,96.7506637573242
4240000,114.999572753906
4280000,97.1450881958008
4320000,104.269371032715
4360000,80.1777420043945
4400000,91.9394912719727
4440000,88.1764678955078
4480000,95.2518920898438
4520000,77.6729431152344
4560000,92.3959045410156
4600000,93.1308364868164
4640000,79.9378890991211
4680000,91.4608612060547
4720000,94.1199722290039
4760000,95.5909652709961
4800000,92.6663208007813
4840000,100.486000061035
4880000,112.995941162109
4920000,97.1742095947266
4960000,108.007537841797
5000000,97.8075866699219
5040000,85.3363342285156
5080000,95.7679061889648
5120000,78.8093795776367
5160000,114.461128234863
5200000,104.184646606445
5240000,96.0162582397461
5280000,108.453605651855
5320000,109.765007019043
5360000,121.193832397461
5400000,128.507949829102
5440000,134.129776000977
5480000,109.978614807129
5520000,125.296989440918
5560000,124.144172668457
5600000,118.809753417969
5640000,129.676330566406
5680000,122.536827087402
5720000,129.687026977539
5760000,131.389144897461
5800000,133.483001708984
5840000,142.509460449219
5880000,135.374740600586
5920000,124.693206787109
5960000,130.804779052734
6000000,143.616485595703
6040000,139.375106811523
6080000,134.612976074219
6120000,131.656967163086
6160000,161.227478027344
6200000,130.707107543945
6240000,137.593017578125
6280000,122.437652587891
6320000,140.823806762695
6360000,144.988647460938
6400000,141.83039855957
6440000,162.43879699707
6480000,135.152618408203
6520000,153.006622314453
6560000,149.372192382813
6600000,160.221160888672
6640000,162.691452026367
6680000,144.174575805664
6720000,156.4013671875
6760000,150.810913085938
6800000,164.9736328125
6840000,143.308181762695
6880000,146.757873535156
6920000,151.26432800293
6960000,141.041137695313
7000000,145.858215332031
7040000,146.045013427734
7080000,132.486129760742
7120000,145.606506347656
7160000,138.588150024414
7200000,155.064025878906
7240000,162.399932861328
7280000,148.8681640625
7320000,163.12174987793
7360000,157.538330078125
7400000,170.36540222168
7440000,178.702621459961
7480000,172.041793823242
7520000,165.225921630859
7560000,174.696517944336
7600000,149.365905761719
7640000,157.01057434082
7680000,173.480575561523
7720000,164.832626342773
7760000,174.595825195313
7800000,170.932098388672
7840000,188.461761474609
7880000,179.020767211914
7920000,175.726684570313
7960000,166.274505615234
8000000,181.724136352539
8040000,190.075927734375
8080000,187.903060913086
8120000,166.492263793945
8160000,167.979827880859
8200000,174.417602539063


==> Datasets/reward.tex <==
40000,-42.310707092285156
80000,-24.43977165222168
120000,-12.628936767578125
160000,-9.789884567260742
200000,-11.489229202270508
240000,-10.947487831115723
280000,-5.8668212890625
320000,-1.060756802558899
360000,-0.09295809268951416
400000,-9.364733695983887
440000,-11.417863845825195
480000,-2.2590222358703613
520000,3.7731170654296875
560000,5.243621349334717
600000,4.800950050354004
640000,-3.325834035873413
680000,10.882420539855957
720000,4.397948265075684
760000,4.775602340698242
800000,20.03204917907715
840000,44.960723876953125
880000,33.24127197265625
920000,33.81075668334961
960000,46.674991607666016
1000000,35.334129333496094
1040000,33.15052032470703
1080000,26.717567443847656
1120000,36.588890075683594
1160000,36.200401306152344
1200000,40.524009704589844
1240000,35.34859848022461
1280000,46.08892822265625
1320000,57.73933410644531
1360000,57.93019485473633
1400000,36.60684585571289
1440000,47.000450134277344
1480000,39.31343078613281
1520000,48.087242126464844
1560000,45.66206741333008
1600000,37.778961181640625
1640000,54.94217300415039
1680000,64.3333969116211
1720000,48.885494232177734
1760000,56.99032974243164
1800000,71.6348876953125
1840000,49.84476852416992
1880000,41.329715728759766
1920000,47.47622299194336
1960000,56.81117630004883
2000000,61.31814956665039
2040000,44.62455749511719
2080000,39.12220764160156
2120000,38.81631088256836
2160000,57.80617141723633
2200000,50.118431091308594
2240000,46.66523361206055
2280000,58.84708786010742
2320000,53.265384674072266
2360000,60.69571304321289
2400000,67.85193634033203
2440000,53.555110931396484
2480000,65.22093963623047
2520000,43.17123794555664
2560000,78.30045318603516
2600000,56.24610137939453
2640000,56.370567321777344
2680000,37.60580825805664
2720000,57.89521408081055
2760000,60.00946807861328
2800000,52.600555419921875
2840000,46.834293365478516
2880000,54.158084869384766
2920000,59.0766487121582
2960000,55.05060577392578
3000000,61.04025650024414
3040000,53.072242736816406
3080000,49.14518737792969
3120000,39.05876541137695
3160000,51.41061782836914
3200000,43.70572280883789
3240000,59.959510803222656
3280000,56.233760833740234
3320000,65.1469955444336
3360000,69.39849853515625
3400000,54.98484420776367
3440000,45.4022102355957
3480000,76.95260620117188
3520000,71.38334655761719
3560000,74.4120864868164
3600000,65.957763671875
3640000,52.8670539855957
3680000,50.4587287902832
3720000,60.27222442626953
3760000,80.02820587158203
3800000,71.12523651123047
3840000,53.10136032104492
3880000,73.64270782470703
3920000,67.38862609863281
3960000,51.30244064331055
4000000,37.17961883544922
4040000,83.03060150146484
4080000,57.25455856323242
4120000,60.2113151550293
4160000,45.621315002441406
4200000,51.64684295654297
4240000,55.60398864746094
4280000,73.13980865478516
4320000,57.94052505493164
4360000,75.42848205566406
4400000,55.16788101196289
4440000,55.29729080200195
4480000,58.42088317871094
4520000,65.1275405883789
4560000,44.83586502075195
4600000,49.51708984375
4640000,60.94932174682617
4680000,60.63264465332031
4720000,60.18584442138672
4760000,45.227508544921875
4800000,53.174591064453125
4840000,40.78917694091797
4880000,58.54615783691406
4920000,59.961246490478516
4960000,36.5650520324707
5000000,68.7611083984375
5040000,62.20183181762695
5080000,77.52417755126953
5120000,62.67420196533203
5160000,62.60142135620117
5200000,77.61597442626953
5240000,42.47330093383789
5280000,74.35955047607422
5320000,67.81304168701172
5360000,68.6348648071289
5400000,94.04110717773438
5440000,68.20396423339844
5480000,67.38330078125
5520000,83.5908432006836
5560000,70.2432861328125
5600000,72.46351623535156
5640000,75.081298828125
5680000,79.16573333740234
5720000,80.34272003173828
5760000,72.87932586669922
5800000,74.55123901367188
5840000,64.2107162475586
5880000,103.74107360839844
5920000,60.26861572265625
5960000,60.84491729736328
6000000,70.87157440185547
6040000,66.74677276611328
6080000,63.73520278930664
6120000,69.77884674072266
6160000,54.60313034057617
6200000,66.4214096069336
6240000,60.12421798706055
6280000,62.923194885253906
6320000,76.69214630126953
6360000,65.90586853027344
6400000,93.88773345947266
6440000,77.45730590820312
6480000,77.7248306274414
6520000,75.22074890136719
6560000,55.91122817993164
6600000,43.38481140136719
6640000,63.94856262207031
6680000,66.5601577758789
6720000,74.88935852050781
6760000,78.60468292236328
6800000,82.23680114746094
6840000,69.3144302368164
6880000,57.682762145996094
6920000,76.00887298583984
6960000,50.480770111083984
7000000,73.40392303466797
7040000,71.87641143798828
7080000,56.80107498168945
7120000,62.624229431152344
7160000,61.19255065917969
7200000,68.19114685058594
7240000,62.88851547241211
7280000,49.6038932800293
7320000,71.9923095703125
7360000,62.410865783691406
7400000,61.043556213378906
7440000,77.63505554199219
7480000,75.76910400390625
7520000,66.04613494873047
7560000,88.18290710449219
7600000,66.0436782836914
7640000,60.45432662963867
7680000,67.03568267822266
7720000,84.35831451416016
7760000,62.123435974121094
7800000,68.69566345214844
7840000,55.04652786254883
7880000,61.546844482421875
7920000,69.16835021972656
7960000,68.58524322509766
8000000,69.9893569946289
8040000,67.30205535888672
8080000,61.022029876708984
8120000,79.31285858154297
8160000,81.03905487060547
8200000,69.77165222167969


==> Datasets/rovpose_set4.tex <==
610.291589,-581.087432,0.218647897
589.056476,-583.685319,0.212747322
573.144769,-574.817153,0.214263452
555.780828,-563.586183,0.214568054
539.233607,-553.321959,0.21459339
525.350440,-545.336450,0.213297397
512.623100,-538.733258,0.211470413
505.851266,-528.417449,0.209457682
499.157818,-511.742521,0.207978369
481.563132,-482.970690,0.207988328
457.789574,-445.743281,0.209128573
431.103931,-399.730525,0.211697161
402.659206,-346.655770,0.215042647
374.274616,-288.739601,0.218593735
346.895888,-226.396237,0.222572616
321.762113,-160.553779,0.225896322
303.064882,-95.579771,0.228693999
295.407774,-38.122947,0.228596517
288.922276,10.727871,0.2266446
282.990288,54.034271,0.223919121
267.782602,94.244469,0.221985351
243.672791,136.180229,0.218727669
211.052842,180.961009,0.216704155
173.298643,224.573993,0.216706694
148.792826,277.005886,0.212563474
136.272348,327.779791,0.205515943
125.562115,372.887400,0.199965268
119.399675,411.289256,0.195413997
115.914920,442.269637,0.195136634
120.036694,465.407670,0.195036286
124.674474,484.004877,0.196668942
130.316268,499.842731,0.198321904
136.651737,513.821875,0.199505368
146.117796,526.262326,0.200315521
158.336415,536.412069,0.200987139
174.556444,544.755378,0.203180147
192.907961,549.622232,0.205377099
211.725978,552.259784,0.207697041
231.061142,551.778569,0.208563636
248.821737,550.668214,0.208091925
266.423638,546.670845,0.206701222
280.592822,537.018499,0.203472119
293.976123,522.552462,0.199418518
305.521754,504.846042,0.195607328
315.321591,486.395772,0.193268965
322.444089,469.458915,0.191943994
327.996069,454.559099,0.190496901
332.659925,444.971293,0.189731659
336.115926,436.727273,0.190767253
339.113746,432.964048,0.192034743
344.424811,434.927815,0.193700316
354.398291,441.755042,0.196582246
367.465440,451.422267,0.199054529
385.063004,463.304962,0.201617648
404.894754,476.490567,0.205103192
429.042712,488.824671,0.20829819
452.068558,502.737137,0.209872787
477.182828,515.488021,0.209713401
505.436658,525.473096,0.209981226
533.845760,535.836281,0.209371877
559.872466,548.949640,0.207480996
583.499691,562.745273,0.205188466
601.289046,575.125465,0.203635829
614.581581,586.060000,0.202995563
627.143118,597.501558,0.202096902
641.431863,610.364687,0.202545403
660.646094,623.725022,0.203114122
680.575402,635.728518,0.204863382
704.998170,647.212392,0.207122573
733.125782,656.674463,0.209689756
763.644874,666.767648,0.21274565
792.999021,675.623383,0.215645723
820.783615,683.029867,0.217044942
843.890562,690.108404,0.218353132
862.239248,698.000025,0.217285287
878.211475,705.954932,0.215747995
891.269734,712.766942,0.212913352
903.485020,716.807419,0.211597722
926.828473,717.586782,0.218676731
948.238850,709.610228,0.22345085
989.261336,704.373087,0.235042714
1019.691799,694.800314,0.238654779



==> Datasets/sac_reward.tex <==
60000,1.979192138
120000,-1.885190606
180000,-1.263238311
240000,12.27098656
300000,-2.380935907
360000,9.625349045
420000,7.966679096
480000,-21.36313629
540000,5.085780621
600000,-18.14911652
660000,21.24854279
720000,20.99489403
780000,3.746331692
840000,36.35178375
900000,18.85031509
960000,20.66321373
1020000,12.52728748
1080000,29.14676857
1140000,18.20649529
1200000,25.52783012
1260000,25.90008926
1320000,3.121369362
1380000,20.05031586
1440000,15.60878277
1500000,23.13263321
1560000,17.37685776
1620000,22.78323746
1680000,16.43714905
1740000,39.98749161
1800000,25.10035896
1860000,33.69886398
1920000,24.04692459
1980000,37.31915665
2040000,38.06237793
2100000,34.08191681
2160000,38.27997208
2220000,32.90043259
2280000,36.63525772
2340000,54.17140961
2400000,46.3651123
2460000,28.95522499
2520000,23.64258194
2580000,31.93526649
2640000,39.42138672
2700000,32.99328613
2760000,34.04442596
2820000,37.24890518
2880000,26.712286
2940000,36.16070557
3000000,32.14263535
3060000,47.40237427
3120000,26.95105553
3180000,37.37760925
3240000,31.4888382
3300000,26.40133286
3360000,31.22958755
3420000,29.77236748
3480000,39.28726959
3540000,32.60351563
3600000,39.12614441
3660000,26.00522232
3720000,34.96710587
3780000,27.51996613
3840000,22.91603279
3900000,33.40974426
3960000,23.84367371
4020000,27.54288483
4080000,41.80489731
4140000,32.68854523
4200000,40.15800858
4260000,33.7983284
4320000,34.88607407
4380000,39.85570526
4440000,24.30379486
4500000,49.74444199
4560000,46.28759003
4620000,38.7240715
4680000,16.36264038
4740000,32.40792847
4800000,32.99863815
4860000,20.91224098
4920000,32.57658768
4980000,27.14886475
5040000,30.81170654
5100000,22.64116859
5160000,37.53476334
5220000,58.01887131
5280000,35.82252121
5340000,32.1248703
5400000,29.75924683
5460000,44.49482346
5520000,28.83917618
5580000,37.17230606
5640000,32.62844467
5700000,27.48688889
5760000,37.17192459
5820000,17.33387375
5880000,35.87513733
5940000,28.95143318
6000000,34.45849228
6060000,37.38916397
6120000,41.84720993
6180000,34.00094223
6240000,12.69916534
6300000,43.89143372
6360000,45.06732941
6420000,27.19661713
6480000,45.84488678
6540000,36.2748642
6600000,15.12757874
6660000,36.85804749
6720000,39.71904373
6780000,41.14693832
6840000,43.19106674
6900000,26.34968948
6960000,21.35266876
7020000,50.92506027
7080000,51.47382736
7140000,42.63674927
7200000,31.71509933
7260000,38.33125687
7320000,27.21670723
7380000,46.46227264
7440000,11.83568573
7500000,13.39327049
7560000,12.08423901

